Small Character Models Match Large Word Models for Autocomplete Under Memory Constraints

Autocomplete is a task where the user inputs a piece of text, termed prompt, which is conditioned by the model to generate semantically coherent continuation. Existing works for this task have primarily focused on datasets (e.g., email, chat) with high frequency user prompt patterns (or focused prompts) where word-based language models have been quite effective. In this work, we study the more challenging open-domain setting consisting of low frequency user prompt patterns (or broad prompts, e.g., prompt about 93rd academy awards) and demonstrate the effectiveness of character-based language models. We study this problem under memory-constrained settings (e.g., edge devices and smartphones), where character-based representation is effective in reducing the overall model size (in terms of parameters). We use WikiText-103 benchmark to simulate broad prompts and demonstrate that character models rival word models in exact match accuracy for the autocomplete task, when controlled for the model size. For instance, we show that a 20M parameter character model performs similar to an 80M parameter word model in the vanilla setting. We further propose novel methods to improve character models by incorporating inductive bias in the form of compositional information and representation transfer from large word models. Datasets and code used in this work are available at https://github.com/UBC-NLP/char_autocomplete.

==> dump.tex <==


\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[height=1.05in, width=1.8in]{images/80M_bertstyle_EM1.pdf}
        %\caption{ExactMatch@1}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[height=1.05in, width=1.8in]{images/80M_bertstyle_EM2.pdf}
        %\caption{ExactMatch@2}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[height=1.05in, width=1.8in]{images/80M_bertstyle_EM3.pdf}
        %\caption{ExactMatch@3}
    \end{subfigure}
    \caption{Improvements of character models of size $80M$ with BERT-style and character pooling over vanilla character model on WikiText-103 validation set.}
    \label{fig:res_bert_charavg_80M}
\end{figure*}



\begin{comment}
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[height=1.05in, width=1.8in]{images/10M_bertstyle_EM1.pdf}
        %\caption{ExactMatch@1}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[height=1.05in, width=1.8in]{images/10M_bertstyle_EM2.pdf}
        %\caption{ExactMatch@2}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[height=1.05in, width=1.8in]{images/10M_bertstyle_EM3.pdf}
        %\caption{ExactMatch@3}
    \end{subfigure}
    \caption{Improvements of character models of sizes $5M$, $10M$ and $20M$ with BERT-style and character pooling.}
    \label{fig:res_bert_charavg_small}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[height=1.25in, width=2.5in]{images/ltransfer_res.pdf}
        %\caption{ExactMatch@1}
    \end{subfigure}%
    \caption{Improvements of character models of sizes $5M$, $10M$ and $20M$ with decoder layer transfer method. The size of the word model is displayed in the plot.}
    \label{fig:res_layertrans}
\end{figure*}
\end{comment}

==> ppl_vs_em_unfinished.tex <==
\pagebreak
\subsection{Theoretical study on difference in Exact Match and Perplexity metric}
\label{sec:theory_em_vs_ppl_diff}
Let us formally study the difference in the information captured by the exact match and the perplexity metric. Assume that the language model is word based and the autocomplete task is to predict only the next word. 
Let us define the Exact Match metric:

\begin{multline}\label{eq:em_defn}
\small
ExactMatch(\hat{x}, x) = \frac{1}{|\mathcal{D}|}  \sum_{j=1}^{|\mathcal{D}|} \sum_{k=1}^{|\mathcal{V}|} 1(x^j_k == 1) \\ 1(\arg\max_l \hat{x}^j_l == k),
\end{multline}

where $1(.)$ denotes the indicator function that produces $1$ if the condition is true, otherwise produces $0$. Let us define the perplexity metric:

\begin{multline}\label{eq:ppl_defn}
Perplexity(\hat{x}, x) = 2^{-\frac{1}{|\mathcal{D}|}  \sum_{j=1}^{|\mathcal{D}|} \sum_{k=1}^{|\mathcal{V}|} x^j_k \times \log(\hat{x}^j_k)}
\end{multline}

Since exponential function is monotonically increasing, we can simplify the previous equation by dropping the exponential. The approximate perplexity score then will be: 
\begin{multline}\label{eq:app_ppl_defn}
Perplexity(\hat{x}, x) \approx -\frac{1}{|\mathcal{D}|}  \sum_{j=1}^{|\mathcal{D}|} \sum_{k=1}^{|\mathcal{V}|} x^j_k \times \log(\hat{x}^j_k)
\end{multline}

If we compare the approximate perplexity score with the exact match score,

\begin{multline}\label{eq:comp_defn}
ExactMatch(\hat{x}, x) ? Perplexity(\hat{x}, x) \\
\frac{1}{|\mathcal{D}|}  \sum_{j=1}^{|\mathcal{D}|} \sum_{k=1}^{|\mathcal{V}|} 1(x^j_k == 1) 1(\arg\max_l \hat{x}^j_l == k) ? \\ -\frac{1}{|\mathcal{D}|}  \sum_{j=1}^{|\mathcal{D}|} \sum_{k=1}^{|\mathcal{V}|} x^j_k \times \log(\hat{x}^j_k) \\
\sum_{k=1}^{|\mathcal{V}|} 1(x^j_k == 1) 1(\arg\max_l \hat{x}^j_l == k) ? - \sum_{k=1}^{|\mathcal{V}|} x^j_k \times \log(\hat{x}^j_k)
\end{multline}

Let us form hypothesis on the nature of distribution underlying $\mathbf{\hat{x}^j}$ and observe how the two scores differ.

\noindent\textbf{\underline{$\mathbf{\hat{x}^j}$ is one-hot distribution}}:
If the model prediction is correct (that is, $1(\arg\max_l \hat{x}^j_l == \arg\max_m x^j_m )$), then the equation~\ref{eq:comp_defn} becomes:
\begin{multline}\label{eq:case1}
\sum_{k=1}^{|\mathcal{V}|} 1(x^j_k == 1) 1(\arg\max_l \hat{x}^j_l == k) ? - \sum_{k=1}^{|\mathcal{V}|} x^j_k \times \log(\hat{x}^j_k) \\
1 ? 0.
\end{multline}

If the model prediction is incorrect, then the equation~\ref{eq:comp_defn} becomes:
\begin{multline}\label{eq:case2}
\sum_{k=1}^{|\mathcal{V}|} 1(x^j_k == 1) 1(\arg\max_l \hat{x}^j_l == k) ? - \sum_{k=1}^{|\mathcal{V}|} x^j_k \times \log(\hat{x}^j_k) \\
0 ? -\log_2 (0).
\end{multline}
 
\noindent\textbf{\underline{$\mathbf{\hat{x}^j}$ is uniform distribution}}: If the model prediction is correct (that is, $1(\arg\max_l \hat{x}^j_l == \arg\max_m x^j_m )$), then the equation~\ref{eq:comp_defn} becomes:
\begin{multline}\label{eq:case3}
\sum_{k=1}^{|\mathcal{V}|} 1(x^j_k == 1) 1(\arg\max_l \hat{x}^j_l == k) ? - \sum_{k=1}^{|\mathcal{V}|} x^j_k \times \log(\hat{x}^j_k) \\
1 ? - \log_2 \frac{1}{|\mathcal{V}|}.
\end{multline}

If the model prediction is incorrect, then the equation~\ref{eq:comp_defn} becomes:
\begin{multline}\label{eq:case4}
\sum_{k=1}^{|\mathcal{V}|} 1(x^j_k == 1) 1(\arg\max_l \hat{x}^j_l == k) ? - \sum_{k=1}^{|\mathcal{V}|} x^j_k \times \log(\hat{x}^j_k) \\
0 ? - \log_2 \frac{1}{|\mathcal{V}|}.
\end{multline}
